Hamiltonian Chaos: From Galactic Dynamics to Plasma Physics

The primary focus of this thesis is the numerical investigation of chaos in Hamiltonian models describing charged particle orbits in plasma, star motions in barred galaxies, and orbits' diffusion in multidimensional maps. We systematically explore the interplay between magnetic and kinetic chaos in toroidal fusion plasmas, where non-axisymmetric perturbations disrupt smooth magnetic flux surfaces, generating complex particle trajectories. Using the Generalized Alignment Index (GALI) method, we efficiently quantify chaos, compare the behavior of magnetic field lines and particle orbits, visualize the radial distribution of chaotic regions, and offer GALI as a valuable tool for studying plasma physics dynamics. We also study the evolution of phase space structures in a 3D barred galactic potential, following successive 2D and 3D pitchfork and period-doubling bifurcations of periodic orbits. By employing the `color and rotation' technique to visualize the system's 4D Poincar\'e surface of sections, we reveal distinct structural patterns. We further investigate the long-term diffusion transport and chaos properties of single and coupled standard maps, focusing on parameters inducing anomalous diffusion through accelerator modes exhibiting ballistic transport. Using different ensembles of initial conditions in chaotic regions influenced by these modes, we examine asymptotic diffusion rates and time scales, identifying conditions suppressing anomalous transport and leading to long-term convergence to normal diffusion across coupled maps. Lastly, we perform the first comprehensive investigation into the GALI indices for various attractors in continuous and discrete-time dissipative systems, extending the method's application to non-Hamiltonian systems. A key aspect of our work involves analyzing and comparing GALIs' with Lyapunov Exponents for systems exhibiting hyperchaotic motion.

==> Thesis_Dedication.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                      %
%     File: Thesis_Dedication.tex                                      %
%     Tex PhD: Thesis.tex                                           %
%                                                                      %
%     Author: H.T. Moges                                          %
%     Last modified :  March 2024                                      %
%                                                                      %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\null\vskip5cm%
\begin{flushright}
     Dedicated to someone special...
\end{flushright}
\vfill\newpage


